Solver-based Gradual Type Migration

Gradually typed languages allow programmers to mix statically and dynamically typed code, enabling them to incrementally reap the benefits of static typing as they add type annotations to their code. However, this type migration process is typically a manual effort with limited tool support. This paper examines the problem of \emph{automated type migration}: given a dynamic program, infer additional or improved type annotations. Existing type migration algorithms prioritize different goals, such as maximizing type precision, maintaining compatibility with unmigrated code, and preserving the semantics of the original program. We argue that the type migration problem involves fundamental compromises: optimizing for a single goal often comes at the expense of others. Ideally, a type migration tool would flexibly accommodate a range of user priorities. We present TypeWhich, a new approach to automated type migration for the gradually-typed lambda calculus with some extensions. Unlike prior work, which relies on custom solvers, TypeWhich produces constraints for an off-the-shelf MaxSMT solver. This allows us to easily express objectives, such as minimizing the number of necessary syntactic coercions, and constraining the type of the migration to be compatible with unmigrated code. We present the first comprehensive evaluation of GTLC type migration algorithms, and compare TypeWhich to four other tools from the literature. Our evaluation uses prior benchmarks, and a new set of ``challenge problems.'' Moreover, we design a new evaluation methodology that highlights the subtleties of gradual type migration. In addition, we apply TypeWhich to a suite of benchmarks for Grift, a programming language based on the GTLC. TypeWhich is able to reconstruct all human-written annotations on all but one program.

==> bibexport.bib-save-2021.09.10_12.38.55 <==


@inproceedings{th:migration,
  author =        {Sam {Tobin-Hochstadt} and Matthias Felleisen},
  booktitle =     {Dynamic Languages Symposium (DLS)},
  title =         {Interlanguage Migration: From Scripts to Programs},
  year =          {2006},
}

@inproceedings{siek:gtlc,
  author =        {Jeremy~G. Siek and Walid Taha},
  booktitle =     {Scheme and Functional Programming Workshop (SW)},
  title =         {Gradual Typing for Functional Languages},
  year =          {2006},
}

@article{wright:soft-typing,
  author =        {Andrew~K. Wright and Robert Cartwright},
  journal =       {{ACM} Transactions on Programming Languages and
                   Systems (TOPLAS)},
  number =        {1},
  pages =         {87--152},
  title =         {A Practical Soft Type System for Scheme},
  volume =        {19},
  year =          {1997},
}

@inproceedings{flanagan:spidey,
  author =        {Cormac Flanagan and Matthew Flatt and
                   Shriram Krishnamurthi and Stephanie Weirich and
                   Matthias Felleisen},
  booktitle =     {ACM SIGPLAN Conference on Programming Language Design
                   and Implementation (PLDI)},
  title =         {Catching Bugs in the Web of Program Invariants},
  year =          {1996},
}

@inproceedings{scheme-to-ml,
  author =        {Fritz Henglein and Jakob Rehof},
  booktitle =     {International Conference on Functional Programming
                   Languages and Computer Architecture (FPCA)},
  title =         {Safe polymorphic type inference for a dynamically
                   typed language: Translating {Scheme} to {ML}},
  year =          {1995},
}

@inproceedings{siek:gti,
  author =        {Jeremy~G. Siek and Manish Vachharajani},
  booktitle =     {Dynamic Languages Symposium (DLS)},
  title =         {Gradual Typing with Unification-based Inference},
  year =          {2008},
}

@inproceedings{rastogi:gti,
  author =        {Aseem Rastogi and Avik Chaudhuri and Basil Hosmer},
  booktitle =     {ACM SIGPLAN-SIGACT Symposium on Principles of
                   Programming Languages (POPL)},
  title =         {The Ins and Outs of Gradual Type Inference},
  year =          {2012},
}

@article{campora:migrating,
  author =        {John~Peter Campora and Sheng Chen and Martin Erwig and
                   Eric Walkingshaw},
  journal =       {Proceedings of the ACM on Programming Languages
                   (PACMPL)},
  number =        {POPL},
  title =         {Migrating Gradual Types},
  volume =        {2},
  year =          {2018},
}

@article{migeed:decidable,
  author =        {Zeina Migeed and Jens Palsberg},
  journal =       {Proceedings of the ACM on Programming Languages
                   (PACMPL)},
  number =        {POPL},
  title =         {What is Decidable about Gradual Types?},
  volume =        {4},
  year =          {2020},
}

@inproceedings{z3maxsmt,
  author =        {Nikolaj Bj{\o}rner and {Anh-Dung} Phan and
                   Lars Fleckenstein},
  booktitle =     {Tools and Algorithms for the Construction and
                   Analysis of Systems (TACAS)},
  title =         {$\nu$Z: An Optimizing {SMT} Solver},
  year =          {2015},
}

@inproceedings{kuhlenschmidt:grift,
  author =        {Andre Kuhlenschmidt and Deyaaeldeen Almahallawi and
                   Jeremy~G. Siek},
  booktitle =     {ACM SIGPLAN Conference on Programming Language Design
                   and Implementation (PLDI)},
  title =         {Toward Efficient Gradual Typing for Structural Types
                   via Coercions},
  year =          {2019},
}

@article{henglein:coercions,
  author =        {Fritz Henglein},
  journal =       {Science of Computer Programming},
  number =        {3},
  pages =         {197--230},
  title =         {Dynamic typing: syntax and proof theory},
  volume =        {22},
  year =          {1994},
}

@inproceedings{siek:refined,
  author =        {Jeremy Siek and Michael Vitousek and Matteo Cimini and
                   John Boyland},
  booktitle =     {Summit oN Advances in Programming Languages (SNAPL)},
  title =         {Refined Criteria for Gradual Typing},
  year =          {2015},
}

@article{herman:space,
  author =        {David Herman and Aaron Tomb and Cormac Flanagan},
  journal =       {Higher-Order and Symbolic Computation (HOSC)},
  number =        {2},
  pages =         {167--189},
  title =         {Space-efficient gradual typing},
  volume =        {23},
  year =          {2011},
}

@phdthesis{greenberg:thesis,
  author =        {Michael Greenberg},
  school =        {University of Pennsylvania},
  title =         {Manifest Contracts},
  year =          {2013},
}

@inproceedings{siek:coercion,
  author =        {Jeremy Siek and Peter Thiemann and Philip Wadler},
  booktitle =     {ACM SIGPLAN Conference on Programming Language Design
                   and Implementation (PLDI)},
  title =         {Blame and Coercion: Together Again for the First
                   Time},
  year =          {2015},
}

@article{smt-adt,
  author =        {Clark Barrett and Iger Shikanian and Cesare Tinelli},
  journal =       {Journal on Satisfiability, Boolean Modeling and
                   Computation},
  number =        {1--2},
  pages =         {21--46},
  title =         {An Abstract Decision Procedure for a Theory of
                   Inductive Data Types},
  volume =        {3},
  year =          {2007},
}

@article{campora:herder,
  author =        {John~Peter Campora and Sheng Chen and
                   Eric Walkingshaw},
  journal =       {Proceedings of the ACM on Programming Languages
                   (PACMPL)},
  number =        {ICFP},
  title =         {Casts and Costs: Harmonizing Safety and Performance
                   in Gradual Typing},
  volume =        {2},
  year =          {2018},
}

@inproceedings{gtlc-mono,
  author =        {Jeremy~G.~Siek and Michael~M. Vitousek and
                   Matteo Cimini and Sam {Tobin-Hochstadt} and
                   Ronald Garcia},
  booktitle =     {European Symposium on Programming (ESOP)},
  title =         {Monotonic References for Efficient Gradual Typing},
  year =          {2015},
}

@article{chen:variational,
  author =        {Sheng Chen and Martin Erwig and Eric Walkingshaw},
  journal =       {{ACM} Transactions on Programming Languages and
                   Systems (TOPLAS)},
  number =        {1},
  title =         {Extending Type Inference to Variational Programs},
  volume =        {36},
  year =          {2014},
}

@inproceedings{vitousek:reticulated,
  author =        {Michael M. Vitousek and Jeremy G. Siek and Jim Baker},
  booktitle =     {Dynamic Languages Symposium (DLS)},
  title =         {Design and Evaluation of Gradual Typing for Python},
  year =          {2014},
}

@inproceedings{greenman:tags,
  author =        {Ben Greenman and Zeina Migeed},
  booktitle =     {ACM SIGPLAN Workshop on Partial Evaluation and
                   Program Manipulation (PEPM)},
  title =         {On the Cost of Type-Tag Soundness},
  year =          {2018},
}

@article{greenman:spectrum,
  author =        {Ben Greenman and Matthias Felleisen},
  number =        {ICFP},
  title =         {A Spectrum of Type Soundness and Performance},
  volume =        {2},
  year =          {2018},
}

@inproceedings{vitousek:runtime,
  author =        {Michael M. Vitousek and Cameron Swords and
                   Jeremy G. Siek},
  booktitle =     {ACM SIGPLAN-SIGACT Symposium on Principles of
                   Programming Languages (POPL)},
  title =         {Big Types in Little Runtime: Open-World Soundness and
                   Collaborative Blame for Gradual Type Systems},
  year =          {2017},
}

@inproceedings{garcia:principal-gradual-types,
  author =        {Ronald Garcia and Matteo Cimini},
  booktitle =     {ACM SIGPLAN-SIGACT Symposium on Principles of
                   Programming Languages (POPL)},
  title =         {Principal Type Schemes for Gradual Programs},
  year =          {2015},
}

@article{miyazaki:dti,
  author =        {Yusuke Miyazaki and Taro Sekiyama and
                   Atsushi Igarashi},
  journal =       {Proceedings of the ACM on Programming Languages
                   (PACMPL)},
  number =        {{POPL}},
  title =         {Dynamic Type Inference for Gradual Hindley–Milner
                   Typing},
  volume =        {3},
  year =          {2019},
}

@article{castagna:perspective,
  author =        {Giuseppe Castagna and Victor Lanvin and
                   Tommaso Petrucciani and Jeremy~G. Siek},
  journal =       {Proceedings of the ACM on Programming Languages
                   (PACMPL)},
  number =        {{POPL}},
  title =         {Gradual Typing: A New Perspective},
  volume =        {3},
  year =          {2019},
}

@inproceedings{thf:typedscheme,
  author =        {Sam {T}obin-{H}ochstadt and Matthias Felleisen},
  booktitle =     {ACM SIGPLAN-SIGACT Symposium on Principles of
                   Programming Languages (POPL)},
  title =         {The Design and Implementation of {T}yped {S}cheme},
  year =          {2008},
}

@inproceedings{guha:flowtypes,
  author =        {Arjun Guha and Claudiu Saftoiu and
                   Shriram Krishnamurthi},
  booktitle =     {European Symposium on Programming (ESOP)},
  title =         {Typing Local Control and State Using Flow Analysis},
  year =          {2011},
}

@inproceedings{chugh:systemd,
  author =        {Ravi Chugh and Patrick~M. Rondon and Ranjit Jhala},
  booktitle =     {ACM SIGPLAN-SIGACT Symposium on Principles of
                   Programming Languages (POPL)},
  title =         {Nested Refinements for Dynamic Languages},
  year =          {2012},
}

@inproceedings{vekris:two-phase-typing,
  author =        {Panagiotis Vekris and Benjamin Cosman and
                   Ranjit Jhala},
  booktitle =     {European Conference on Object-Oriented Programming
                   (ECOOP)},
  title =         {Trust, but Verify: Two-Phase Typing for Dynamic
                   Languages},
  year =          {2015},
}

@inproceedings{anderson:inference,
  author =        {Christopher Anderson and Paola Giannini and
                   Sophia Drossopoulou},
  booktitle =     {European Conference on Object-Oriented Programming
                   (ECOOP)},
  title =         {Towards Type Inference for {JavaScript}},
  year =          {2005},
}

@inproceedings{chandra:static-js,
  author =        {Satish Chandra and Colin S. Gordon and
                   Jean{-}Baptiste Jeannin and Cole Schlesinger and
                   Manu Sridharan and Frank Tip and Young{-}Il Choi},
  booktitle =     {ACM SIGPLAN Conference on Object Oriented
                   Programming, Systems, Languages and Applications
                   (OOPSLA)},
  title =         {Type inference for static compilation of
                   {JavaScript}},
  year =          {2016},
}

@inproceedings{wies:errors,
  author =        {Zvonimir Pavlinovic and Tim King and Thomas Wies},
  booktitle =     {ACM SIGPLAN Conference on Object Oriented
                   Programming, Systems, Languages and Applications
                   (OOPSLA)},
  title =         {Finding Minimum Type Error Sources},
  year =          {2014},
}

@phdthesis{flanagan-thesis,
  author =        {Cormac Flanagan},
  school =        {Rice University},
  title =         {Effective Static Debugging via Componential Set-based
                   Analysis},
  year =          {1997},
}

@inproceedings{bard:thorn,
  author =        {Bard Bloom and John Field and Nathaniel Nystrom and
                   Johan {\"{O}}stlund and Gregor Richards and
                   Rok Strni{\v{s}}a and Jan Vitek and Tobias Wrigstad},
  booktitle =     {ACM SIGPLAN Conference on Object Oriented
                   Programming, Systems, Languages and Applications
                   (OOPSLA)},
  title =         {Thorn: Robust, Concurrent, Extensible Scripting on
                   the {JVM}},
  year =          {2009},
}

@inproceedings{furr:drubyoopsla,
  author =        {Michael Furr and {Jong-hoon} David An and
                   Jeffrey~S. Foster},
  booktitle =     {ACM SIGPLAN Conference on Object Oriented
                   Programming, Systems, Languages and Applications
                   (OOPSLA)},
  title =         {Profile-Guilding Static Typing for Dynamic Scripting
                   Languages},
  year =          {2009},
}

@inproceedings{rubydust,
  author =        {{Jong-hoon}~David An and Avik Chauduri and
                   Jeffrey~S. Foster and Michael Hicks},
  booktitle =     {ACM SIGPLAN-SIGACT Symposium on Principles of
                   Programming Languages (POPL)},
  title =         {Dynamic Inference of Static Types for Ruby},
  year =          {2011},
}

@mastersthesis{saftoiu:jstrace,
  author =        {Claudiu Saftoiu},
  school =        {Brown University},
  title =         {{JS}Trace: Run-time type discovery for {JavaScript}},
  year =          {2010},
}

@inproceedings{red:inferdl,
  author =        {Milod Kazerounian and Brianna~M. Ren and
                   Jeffrey~S. Foster},
  booktitle =     {Dynamic Languages Symposium (DLS)},
  title =         {Sound, Heuristic Type Annotation Inference for
                   {Ruby}},
  year =          {2020},
}

@inproceedings{ren:hummingbird,
  author =        {Brianna M. Ren and Jeffrey S. Foster},
  booktitle =     {ACM SIGPLAN Conference on Programming Language Design
                   and Implementation (PLDI)},
  title =         {Just-in-Time Static Type Checking for Dynamic
                   Languages},
  year =          {2016},
}

@inproceedings{hellendoorn:dlti,
  author =        {Hellendoorn, Vincent J. and Bird, Christian and
                   Barr, Earl T. and Allamanis, Miltiadis},
  booktitle =     {ACM SIGSOFT Symposium on the Foundations of Software
                   Engineering (FSE)},
  title =         {Deep Learning Type Inference},
  year =          {2018},
}

@inproceedings{nl2type,
  author =        {Malik, Rabee Sohail and Patra, Jibesh and
                   Pradel, Michael},
  booktitle =     {International Conference on Software Engineering
                   (ICSE)},
  title =         {NL2Type: Inferring JavaScript Function Types from
                   Natural Language Information},
  year =          {2019},
}

@inproceedings{pradel:typewriter,
  author =        {Pradel, Michael and Gousios, Georgios and Liu, Jason and
                   Chandra, Satish},
  booktitle =     {Joint Meeting of the European Software Engineering
                   Conference (ESEC) and the ACM SIGSOFT Symposium on
                   the Foundations of Software Engineering (FSE)},
  title =         {TypeWriter: Neural Type Prediction with Search-Based
                   Validation},
  year =          {2020},
}

@inproceedings{wei:lambdanet,
  author =        {Jiayi Wei and Maruth Goyal and Greg Durrett and
                   Isil Dillig},
  booktitle =     {International Conference on Learning Representations
                   (ICLR)},
  title =         {{LambdaNet}: Probabilistic Type Inference using Graph
                   Neural Networks},
  year =          {2020},
}

@inproceedings{grmtools,
  author =        {Lukas Diekmann and Laurence Tratt},
  booktitle =     {European Conference on Object-Oriented Programming
                   (ECOOP)},
  title =         {Don't Panic! Better, Fewer, Syntax Errors for {LR}
                   Parsers},
  year =          {2020},
}


